A Survey on Deep Domain Adaptation for LiDAR Perception

Scalable systems for automated driving have to reliably cope with an open-world setting. This means, the perception systems are exposed to drastic domain shifts, like changes in weather conditions, time-dependent aspects, or geographic regions. Covering all domains with annotated data is impossible because of the endless variations of domains and the time-consuming and expensive annotation process. Furthermore, fast development cycles of the system additionally introduce hardware changes, such as sensor types and vehicle setups, and the required knowledge transfer from simulation. To enable scalable automated driving, it is therefore crucial to address these domain shifts in a robust and efficient manner. Over the last years, a vast amount of different domain adaptation techniques evolved. There already exists a number of survey papers for domain adaptation on camera images, however, a survey for LiDAR perception is absent. Nevertheless, LiDAR is a vital sensor for automated driving that provides detailed 3D scans of the vehicle's surroundings. To stimulate future research, this paper presents a comprehensive review of recent progress in domain adaptation methods and formulates interesting research questions specifically targeted towards LiDAR perception.

==> tables/applications.tex <==
% !TEX root = ../root.tex

\begin{table}
  \centering
  \caption{
    \textbf{\acs{DA} Applications}:
    TODO Descriptive Caption
  }
  \label{tab:applications}

  \begin{tabularx}{\linewidth}{ll}
    \toprule
    Application & Papers \\
    \midrule

    \simtoreal{} & \cite{Saleh2019ICCVWorkshop}, \cite{Sallab2019ICMLWORK}, \cite{Sallab2019NIPSWORK}, \cite{Zhao2021AAAI}, \cite{Shan2020ArXiv} \\

    \weathertoweather{} & - \\

    \daytonight{} & \cite{Jaritz2020CVPR} \\

    \countrytocountry{} & \cite{Jaritz2020CVPR} \\

    \sensortosensor{} & \cite{Langer2020IROS}, \cite{Shan2020ArXiv}, \cite{Rist2019IV} \\

    \datasettodataset{} & \cite{Saleh2019ICCVWorkshop}, \cite{Alonso2020ArXiv}, \cite{Langer2020IROS}, \cite{Jaritz2020CVPR}, \cite{Jiang2020ArXiv}, \cite{Yi2020ArXiv} \\

    \midrule

    \multicolumn{2}{l}{TODO: Please add the following papers and update the datasets} \\
    \multicolumn{2}{l}{SqueezeSegV2~\cite{Wu2019ICRA-SqueezeSegV2}, SF-UDA3D~\cite{Saltori20203DV}, \cite{Wang2019ICCVWORK}, \cite{Elhadidy2020NILES}, \cite{Zhao2019NIPS}} \\

    \multicolumn{2}{l}{The following are not really in DA context, I will leave them out} \\
    \multicolumn{2}{l}{\cite{Triess2019IV}, \cite{Piewak2019ITSC}} \\

    \bottomrule
  \end{tabularx}

\end{table}


==> tables/datasets.tex <==
% !TEX root = ../root.tex

\begin{table}
  \centering
  \caption{
    \textbf{LiDAR Datasets used for Domain Adaptation}:
    Annotation:
    BB~-~3D bounding boxes,
    TI~-~tracking ids,
    PS~-~point-wise semantics,
    IN~-~point-wise instance ids
  }
  \label{tab:datasets}

  \begin{tabularx}{\linewidth}{@{\hskip 0.6em}l@{\hskip 0.6em}l@{\hskip 0.6em}c@{\hskip 0.6em}c@{\hskip 0.6em}p{1.4cm}}
    \toprule
    Dataset &
    % \acs{lidar} Resolution &
    Frames &
    Annotation &
    Classes &
    \acs{lidar} \acs{DA} Papers \\
    \midrule

    % KITTI
    % Sensor: 1 x Velodyne HDL-64E, mounted on root of vehicle
    % classes: car, van, truck, pedestrian, person (sitting), cyclist, tram and misc
    % Annotations of dynamic objects that lie in the camera's field of view
    \kitti{}~\cite{Geiger2012CVPR} &
    % \multirow{2}{*}{64~\!@\!~10~\!Hz ($\times$1)} &
    \multirow{2}{*}{43,552} &
    BB \!+\! TI &
    8 &
    \cite{Yi2020ArXiv},\cite{Saleh2019ICCVWorkshop} \\

    % SemanticKITTI
    % Sensor: 1 x Velodyne HDL-64E, mounted on roof
    % Based on the KITTI Vision Odometry Benchmark~\cite{Geiger2012CVPR}
    \semantickitti{}~\cite{Behley2019ICCV} &
    % &
    &
    PS \!+\! IN &
    28 &
    \cite{Jiang2020ArXiv},\cite{Langer2020IROS},\cite{Jaritz2020CVPR} \\

    % nuScenes
    % 1.4M boxes, 1.1B points
    % 1000 scenes of 20s each
    % Two diverse cities: Boston, Singapore (left vs. right hand traffic)
    \nuscenes{}~\cite{Caesar2020CVPR} &
    % 32~\!@\!~20~\!Hz ($\times$1) &
    390,000 &
    PS \!/\! BB &
    32 \!/\! 23 &
    \cite{Yi2020ArXiv},\cite{Langer2020IROS},\cite{Jaritz2020CVPR} \\

    % SemanticPOSS
    % Sensor: Pandora (Hesai), 40 channels, LiDAR + camera
    % instance label for (people, car, rider)
    % Data recorded on campus environment
    \semanticposs{}~\cite{Pan2020IV} &
    % 40 ($\times$1) &
    2,988 &
    PS \!/\! IN &
    14 \!/\! 3 &
    \cite{Jiang2020ArXiv},\cite{Alonso2020ArXiv} \\

    % SemanticUSL
    % Sensor: Ouster OS1-64 Lidar
    % For DA research with SemanticKITTI~\cite{Behley2019ICCV} and SemanticPOSS~\cite{Pan2020IV}.
    \semanticusl{}~\cite{Jiang2020ArXiv} &
    % 64 ($\times$1) &
    16,578 \!/\! 1,200 &
    - \!/\! PS &
    - \!/\! 28 &
    \cite{Jiang2020ArXiv} \\

    % Paris-Lille-3D
    % Sensor: 1 x Velodyne HDL-32E LiDAR, 30 degrees tilt to horizontal
    % The frames are complete scenes of accumulated LiDAR sweeps.
    % \parislille{}~\cite{Roynard2017IJRR} &
    % 32 ($\times$1) &
    % 3 &
    % PS &
    % 50 &
    % ... \\

    % A2D2
    % Sensors are tilted
    % Semantics: all points, Box: in field of view of front camera
    \audi{}~\cite{Geyer2020A2D2} &
    % 16~\!@\!~10~\!Hz ($\times$5) &
    % 390,000 \!/\! 41,280 \!/\! 12,499 &
    % - \!/\! PS \!/\! BB &
    % - \!/\! 38 \!/\! 14 &
    41,280 \!/\! 12,499 &
    PS \!/\! BB &
    38 \!/\! 14 &
    \cite{Jaritz2020CVPR} \\

    % Waymo Dataset
    % Sensors: 1 long-range, 4 short-range
    % An domain adaptation benchmark is included
    \waymo{}~\cite{Sun2020ArXiv} &
    % @\!~10~\!Hz ($\times$5) &
    390,000 &
    BB \!+\! TI &
    4 &
    \cite{Yi2020ArXiv} \\

    % \midrule
    %
    % \todoCR{Can you please specify this dataset}
    % % LIBRE
    % % Controlled scenes, adverse weather, multiple sensors
    % \libre{}~\cite{Carballo2020IV} &
    % TODO &
    % TODO &
    % TODO &
    % TODO &
    % - \\
    %
    % % DENSE
    % \dense{}~cite &
    % TODO &
    % TODO &
    % TODO &
    % TODO &
    % - \\

    \midrule

    % CARLA
    % Different sensor models can be simulated with the CARLA framework
    \carla{}~\cite{Dosovitskiy2017CARLA} &
    % custom &
    custom &
    custom &
    $\sim$22 &
    \cite{Saleh2019ICCVWorkshop} \\

    % GTA
    % has no reflectivity information
    \gta{}~\cite{Yue2018ICMR} &
    % custom &
    custom &
    custom &
    $\sim$16 &
     \\

    \bottomrule
  \end{tabularx}

\end{table}


==> tables/sota_overview_deprecated.tex <==
% !TEX root = ../root.tex

\begin{table*}
  \centering
  \caption{
    \textbf{Domain Adaptation Methods for LiDAR Perception}:
    TODO Descriptive Caption
    (Legend:
    $^{a}$Category: DIF -- domain invariant feature learning, DM -- domain mapping, NS -- normalization statistics;
    $^{b}$Use-Cases: D2D -- dataset to dataset, D2N -- day to night, C2C -- country to country, S2R -- simulation to real-world;
    $^{c}$Perception Tasks: detect -- object detection, semseg -- semantic segmentation;
    $^{d}$Metrics: IoU -- intersection over union, AP -- average precision, ACC -- accuracy, CD -- Chamfer Distance
    )
  }
  \label{tab:uda_overview}

  \begin{tabularx}{\linewidth}{l x{0.07\linewidth} x{0.07\linewidth} x{0.07\linewidth} p{0.12\linewidth} p{0.09\linewidth} p{0.1\linewidth} p{0.07\linewidth} p{0.07\linewidth}}
    \toprule
    Paper & Category$^{a}$ & Use-Cases$^{b}$ & Perception Tasks$^{c}$ & Datasets & UDA model & Perception Model & Metrics$^{d}$ & UDA Baselines \\
    \midrule

    Jaritz~\etal~\cite{Jaritz2020CVPR} & DIF & D2N, C2C, D2D & semseg & nuScenes, SemanticKITTI, A2D2 & multimodal & integrated & IoU & MinEnt~\cite{Vu2019CVPR}, Deep logCORAL~\cite{Morerio2018ICLR} \\

    Jiang~\etal~\cite{Jiang2020ArXiv} & DIF & D2D & semseg & SemanticKITTI, SemanticPOSS, SemanticUSL & generative & integrated (SalsaNext~\cite{Cortinhal2020ArXiv}) & IoU & CyCADA~\cite{Hoffman2019ICML} \\

    Yi~\etal~\cite{Yi2020ArXiv} & DIF & D2D & semseg & Waymo, nuScenes, KITTI & sparse voxel completion & sparse voxel labeling & IoU, CD & FeaDA~\cite{Chen2017ICCV}, OutDA~\cite{Tsai2018CVPR} \\

    Saleh~\etal~\cite{Saleh2019ICCVWorkshop} & DM & D2D & detect & CARLA, KITTI & CycleGAN \cite{Zhu2017ICCV-CycleGAN} & YOLOv3 \cite{Redmon2018ArXiv-YOLOv3} & AP & - \\

    Alonso~\etal~\cite{Alonso2020ArXiv} & DM / (NS?) & D2D & semseg & SemanticKITTI, I3A, ParisLille, SemanticPOSS & augmentation & 3D-MiniNet \cite{Alonso2020IROS-MiniNet3D} & IoU & MinEnt, AdvEnt~\cite{Vu2019CVPR}, MaxSquare~\cite{Chen2019ICCV} \\

    Langer~\etal~\cite{Langer2020IROS} & DM & D2D & semseg & nuScenes, SemanticKITTI & resampling & RangeNet++ \cite{Milioto2019IROS-RangeNet++} & IoU, ACC & - \\

    Wu~\etal~\cite{Wu2019ICRA-SqueezeSegV2} & ? (TODO) & S2R & semseg & GTA-V, KITTI & geodesic correlation alignment & SqueezeSegV2 & IoU & SqueezeSeg \\

    Wang~\etal~\cite{Wang2019ICCVWORK} & ? (TODO) & ? (TODO) & detect & KITTI, nuScenes & feature alignment & Complex-YOLO, VoxelNet, SECOND & AP & - \\

    \bottomrule
  \end{tabularx}

\end{table*}

